Developing the Theory of Flux Limits from $\gamma$-Ray Cascades

Dark matter annihilation and other processes may precipitate a flux of diffuse ultra-high energy $\gamma$-rays. These $\gamma$-rays may be observable in present day experiments which observe diffuse fluxes at the GeV scale. Yet the universe is presently opaque to $\gamma$-rays above 10 TeV. It is generally assumed that cascade radiation is observable at all high energies, however the disparity in energy from production to observation has important consequences for theoretical flux limits. We detail the physics of cascade radiation development and consider the influence of energy and redshift scale on arbitrary flux limits that result from electromagnetic cascade.

==> Makefile <==
all: Cascade.pdf

Cascade.dvi: Cascade.tex \
	cascade50TeV.eps cascade100TeV.eps \
	cascade500TeV.eps cascade1000TeV.eps \
	 cascade.eps cascadesteps.eps
	latex $<

Cascade.ps: Cascade.dvi
	dvips -t letter -o $@ $<

Cascade.pdf: Cascade.ps
	ps2pdf $< $@


clean:
	rm -f *.pdf *.ps *.dvi

